SMT Solving for Vesicle Traffic Systems in Cells

In biology, there are several questions that translate to combinatorial search. For example, vesicle traffic systems that move cargo within eukaryotic cells have been proposed to exhibit several graph properties such as three connectivity. These properties are consequences of underlying biophysical constraints. A natural question for biologists is: what are the possible networks for various combinations of those properties? In this paper, we present novel SMT based encodings of the properties over vesicle traffic systems and a tool that searches for the networks that satisfies the properties using SMT solvers. In our experiments, we show that our tool can search for networks of sizes that are considered to be relevant by biologists.

==> bio.tex <==
%Again about two pages long
%
In this section, we will describe the model of VTSs and the properties
relevant to the biologists.

\textbf{The cell as a transport graph:} We consider a cell to be a
collection of compartments (nodes) and vesicles (edges), thus defining
a transport graph.
%
Compartments represent the large membrane-bound organelles, which are
connected by constant fluxes of small transport vesicles.
%
Every compartment or vesicle has a set of molecules associated with
it.
%
These include SNAREs and other biomolecules that regulate membrane
traffic, or that play the role of passive cargo.
%
Here we consider an abstract set of molecules and do
not explicitly associate them with particular protein varieties.\textbf{But consider them to be either of  
the two categories Q and R.}
\textbf{Molecular flows and steady state:} The total amount of each
molecular type on each compartment can increase or decrease: this is
due to gain or loss of that molecular type driven by incoming or
outgoing vesicles.
%
Each edge is thus associated with a flux of all the molecular types
carried by the corresponding vesicle.
%
We assume the cell is in a steady state where each compartments
composition does not vary over time, meaning that all incoming and
outgoing fluxes are balanced for each molecular type at each
compartment; this is the \textit{stability condition}.

\textbf{Vesicle targeting driven by molecular interactions:} The model
specification includes a description of how molecular properties
influence vesicle transport.
%
A vesicle can only contain a set of molecules that are present
on its source compartment.
%
Once a vesicle has budded out of the source, the molecules it carries
determine its properties.
%
In particular, for any given pair of a vesicle and a compartment, the
set of molecules that label the former and latter determine whether
the vesicle will fuse to that compartment.
%
Biophysically, fusion requires a direct physical interaction between
at least one molecular type on the vesicle and one molecular type on
the compartment.
%
The list of molecular pairs that can drive a fusion event is given an
a fusion pairing matrix. \textbf{For convenience, we divide Q and R SNAREs evenly 
and allow only opposite types to become a pair.}

\textbf{Molecular regulation:} The final layer of our framework
involves how the molecules are regulated.
%
We assume that for fusion to occur, the pair of molecular types
involved on the vesicle and compartment must both be in an
“active” state.
%
Whether these molecules are active or inactive depends on the
remaining molecules found on the vesicle or compartment, respectively.
%
This embodies the biological fact that other molecules can regulate the
fusion-driving molecules.
%
VTSs also require that if molecule is involved in fusion of some
vesicle and compartment, it must not be possible that the molecule 
can potentially fuse with some molecule in some other compartment.
%

We test many different versions of molecular
regulation.
%
Most generally, the activity state of a given molecule can be a
Boolean function of all the molecular types on a compartment or vesicles.
We have also tested a particularly simple regulation mechanism in which two
molecules that can pair to drive fusion inhibit one another; this is the \textit{pairing inhibition}.
%
This is motivated by the idea that pairing must generate an inactive
bi-molecular complex.

\textbf{Synthesis:} We now combine all the above ingredients.
%
Given a particular
transport graph, a particular labeling of all the compartments and edges,
a particular fusion pairing matrix, and a particular regulatory model we do
the following.
\begin{enumerate}
\item We determine which molecules are ``active" on every
compartment or vesicle.
\item or every vesicle fusing to a compartment, we
determine whether there exists an active pair (one molecule on the vesicle,
one on the compartment) which drives that fusion event.
\item For every vesicle-compartment pair where the vesicle does not fuse to the
compartment, we verify that there is no pairing of active molecules on the
vesicle and compartment that could drive their fusion.
\item We verify that every molecular type entering a compartment also leaves the compartment,
and also that every molecular type entering a set of compartments also
leaves that set.
%
This tells us that the
particular graph and molecular labeling does represent an allowed steady
state configuration of a VTS.
\end{enumerate}
%The fusion is a process where SNAREs on the vesicles target compartment is driven by the zipping together of vesicle
%and compartment SNAREs [8, 9].
%The SNAREs can be 
%Typically a Q-SNARE triple-helix is confined to one mem-
%brane surface (e.g the compartment), while an R-SNARE single helix is confined to its fusion
%partner (e.g. the vesicle). When these two types of SNAREs are in close proximity they zip
%together into a four-helix bundle, forcing the vesicle to fuse with the compartment. There are
%many types of Q-SNAREs and R-SNAREs spread between different vesicles and compart-
%ments. Across eukaryotes, there are 20 broad SNARE varieties, though individual species can
%contain higher numbers (humans have 41) [12]. Only certain Q and R-SNARE combinations
%can zip into complexes, regulating precisely which vesicles fuse with which targets. For our
%analysis, we consider a Q-SNARE triple helix as a single complex and the R-SNARE as its cog-
%nate partner. We refer to zipping as SNARE pairing.

\begin{itemize}
\item \srivas{Detailed BIO to Graph problem}
\end{itemize}


Given the above conditions, the biologists search for VTSs that are
not $k$-connected, i.e., every pair of compartments remain reachable
after dropping $k-1$ vesicles.
%
It has been observed in nature, most VTSs are 3-connected.
%
It raised the natural question what are the properties of VTSs
that are not 3-connected.
%
To study them, we have build a tool that finds VTSs that are not
$k$-connected from some $k$.

\ankit{Maximum connectivity [LGC, Least guarantee connectivity] and minimal connective [LRC (least required connectivity)] (rather than necc and suff cond) required by the graph.}

\input{pm-1-matrix}

\begin{example}
%
In figure~\ref{fig:M1}, we present a VTS that has 3
compartments and 8 molecules, and corresponding pairing matrix that
describes the fusion dependency.
%
Molecules are numbered 0-7.
%
In the VTS, labels consists of sting of molecule ids and overline
over an id indicates that the molecule is active.
%
This VTS is an example of version where every present molecule on
the node is active and activity of the molecules on the
edges are controlled by presence of the other molecules.
%
On the right side of the figure, we present pairing matrix.
%
An entry 1 represents pairing between molecules and
entry $\times$ represents no pairing.
% rectangles colored $\times$ one represents don't cares.
%
Everywhere in the graph the flux is maintained, i.e.,
every molecule is coming back to it's source node in a cycle.
%
The graph follows the fusion rules as discussed earlier and
is a 3-connected graph.
\ashu{R Q molecule types are not discussed anywhere.}
\end{example}

%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> cz-comparision.tex <==
\begin{figure}[t]
  \centering
\begin{tikzpicture}
  \begin{axis}[
    xbar,
    y axis line style = { opacity = 0 },
    axis x line       = none,
    tickwidth         = 0pt,
    enlarge y limits  = 0.32,
    enlarge x limits  = 0.04,
    symbolic y coords = {Version F, Version E, Version C, Version A},
    nodes near coords,
    legend pos=outer north east,
  ]
  \legend{CBMC, Z3}
  \addplot coordinates { (3053.8,Version A)         (500.03,Version C)
                         (890.84,Version E)  (2482.71,Version F) };
  \addplot coordinates { (7.7,Version A)         (7.60,Version C)
                         (10.27,Version E)   (33.36,Version F)  };  
  \end{axis}
\end{tikzpicture}  
  \caption{CBMC Vs Z3 encoding for N $\equal$ 5 (in secs)}
  \label{fig:cz-comp}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> intro.tex <==
%Total two pages

%\begin{itemize}
%\item \mukund{BIO motivation}

The conservation of basic molecular processes across all living cells,
including the genetic code, suggests that life on Earth arose only
once: all extant organisms are presumed to trace their lineages back
to a last universal common ancestor (LUCA).
%
However, there are still vast differences in cellular and molecular
architecture among the three kingdoms of life: bacteria, archaea, and
eukaryotes~\cite{embley2006eukaryotic}.
%
Eukaryotic cells have larger genomes and have more complex cellular
architectures than the prokaryotic bacteria and archaea.
%
In particular, the cytoplasm of all eukaryotic cells is broken up into
distinct membrane-bound locations known as organelles: the nuclear
membrane, endoplasmic reticulum (ER), Golgi apparatus, vacuoles and
lysosomes are examples of these.
%
Cargo is moved between these organelles in small membrane-bound
transporters known as vesicles \cite{stenmark2009rab}.

This organization resembles a transport logistics network, and is
commonly known as the membrane traffic system.
%
Membrane traffic underpins nearly every aspect of eukaryotic cellular
physiology, including human cellular physiology.
%
Defects in membrane traffic lead to a variety of disorders or even
cell death \cite{stenmark2009rab}.
%
Understanding how membrane traffic functions is therefore one of the
central challenges of cell biology.
%
Some progress has been made, as cell biologists have assembled a
“parts list” of molecules that drive vesicle
traffic~\cite{dacks2007evolution}.
%
The essential processes involve the creation of vesicles loaded with
cargo from source organelles, known as “budding”, and the depositing
of those vesicles and cargo into target organelles, known as “fusion”
\cite{munro2004organelle}.
%
Budding is regulated by proteins known as coats and adaptors that
select cargo.
%
Fusion is regulated by proteins known as SNAREs and tethers, that
ensure that vesicles fuse to the correct target
\cite{mani2016stacking}.
%
Although we know a great deal about molecular-level details, there has
been very little work done on how such processes are integrated across
scales to build the entire vesicle traffic system (VTS).
%
We have recently attempted to use ideas of graph theory to address
this question \cite{mani2016stacking,shukla}.

The SNARE proteins and the constraints that SNARE-to-SNARE regulations
impose on feasibile behaviors of VTSs are the focus of
our current work.
%
Abstractly, we can think of these proteins as labels that are
collected from the source compartment and taken to the target
compartment on vesicles.
%
There is a corresponding set of label molecules on the target compartments.
%
If the two sets of labels (on vesicles and targets) are compatible,
then the vesicle will fuse.
%
The question is: does this physical picture place any constrains on
the global topology of the traffic graph? We have previously shown
that one informative constraint is graph connectivity \cite{shukla}.
%
The intricacies of SNARE regulation are largely unknown.
%
How stringent SNARE regulation is can determine whether graph
topologies of particular level of connectivity are biologically
realizable.
%
For example, if SNAREs are completely unregulated and thus always
active, they cannot be used to generate a traffic network.
%
If these SNAREs are regulated by relatively simple rules then only
highly connected traffic networks can be generated using them.
%
The question is can we work toward a predictive analytical framework
of VTSs?

The analysis of VTSs is a difficult problem because
of the combinatorial scaling of possible traffic topologies and
regulatory rules.
%
Previous analyses of VTSs dealt with this combinatorial explosion by
using a sampling approach: simulating randomly generated regulatory
rules and taking averages over many samples~\cite{mani2016stacking}.
%
The outcome of such simulations is necessarily statistical rather than
rigorous and precise.
%
To make definite predictions about VTS topologies, we need to
efficiently check useful system properties over all possible graphs
and all possible variations of rules, preferably without enumerating
them.
%
Formal verification tools, such as model checkers
\cite{clarke1996symbolic, biere2003bounded, clarke2008birth,
cimatti2000nusmv, holzmann1997model} and SAT solvers
\cite{moskewicz2001chaff,een2004extensible} serve precisely this
purpose.
%
These tools encode the problem symbolically, and check various
properties without explicit enumeration of the graphs up to large but
finite size of the models.

%These tools are central to formal verification methods in computer science, and are increasingly being applied to understand biological systems, including gene regulatory networks [16-18]. 

In a recent work, we employed the model checker CBMC \cite{CKY03,
ckl2004} meant to analyze ANSI C programs for studying this problem.
%
In this work, VTSs and SNARE regulations were modeled as C code mostly
using arrays to represent graphs and boolean tables.
%
Queries about graph connectivity requirements for different variations
of SNARE Regulations were modeled as logical assertions to be checked
by the model checker.
%
CBMC uses its own built-in encodings to reduce the analysis problem to
boolean satisfiability problem which is solved using SAT solvers.
%
This work was successful in demonstrating the feasibility of this
technology to this domain.
%
However, the scalability of this approach was limited (up to VTSs
with 7-8 nodes) due to the following reasons:
\begin{enumerate}
\item The encoding used to model VTSs was not completely fine-tuned
to the structure of the problem.
\item The queries to be solved involve quantified formulas, i.e., we
needed to solve queries of the form ``\emph{for all} graphs does there
\emph{exist} SNARE regulation constraints that satisfy biological
steady state.
\end{enumerate} As CBMC does not directly support solving such
quantified formulas, we had to use a technique that combined
non-determinism and partial enumeration that is not as
efficient.\newline

%
In this paper, we have developed a novel SAT encoding for
searching a VTS that satisfy the given properties.
%
We improved the encoding of some of the conditions for VTSs.
%
In the earlier implementation, reachability was encoded by
enumeration of paths.
%
In our encoding, we have recursively defined the reachability condition
such that that we avoid the exponential enumeration.
%
We have also encoded $k$-connectivity in the similar fashion and
avoided a blowup in the formula size.
%

We have implemented the encoding using Z3~\cite{z3} python API and searched for
VTS satisfying various properties upto size 14-18 nodes as compare
earlier tool that could only search graph upto size 7-8 nodes.
%
Since most VTSs in the cells are of 10 compartments,
our tool will be useful for biologists to study VTSs.
%
Furthermore, our encoding supports several variations of
the conditions.\newline

The following are the contributions of this work:
\begin{itemize}
\item We have added novel encoding reachability and 3-4 connectivity
\item Direct encoding into the SAT solver
\item A user friendly and scalable tool based on well known SMT solver Z3
\end{itemize}

%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> tbl-qf1-graph.tex <==
\begin{table}[t]
  \centering
  \begin{tabular}[t]{|c|c|c|c|c|c|c|c|c|}\hline
    {\multirow{2}{*} \textbf{Size}}  & \multicolumn{2}{c|}{\textbf{Variant A}} & \multicolumn{2}{c|}{\textbf{Variant C}} & \multicolumn{2}{c|}{\textbf{Variant D}}  &  \multicolumn{2}{c|}{\textbf{Variant F}} \\\hline
   
   \cline{2-9}
    {} & {\textbf{A'tool}} & {\textbf{O'cbmc}} & {\textbf{A'tool}} & {\textbf{O'cbmc}} & {\textbf{A'tool}} & {\textbf{O'cbmc}} & {\textbf{A'tool}} & {\textbf{O'cbmc}} \\\hline
    
    2 & !0.085 & !2.43 & 0.15 & 2.12 & !0.13 & !1.89 & 0.35 & 5.12 \\\hline
    3 & !0.54 & !8.04 & 0.95  & 7.65 & 0.62 & 7.66  & 1.36 & 23.94\\\hline
    4 & !2.57 & !297.93 & 2.33 & 22.74 & 2.85 & 48.35  & 4.81 & 123.34\\\hline
    5 & !7.7 & !3053.8 & 7.60 & 500.03 & 10.27 & 890.84 & 33.36  & 2482.71 \\\hline
    6 & !22.98 & M/O & 19.52 & M/O & 30.81 & M/O  & 147.52 & M/O\\\hline
    7 & !57.07 & M/O & 81.89 & M/O & 82.94 & M/O & 522.26  & M/O \\\hline
    8 & !164.14 & M/O & 630.85 & M/O & 303.19 & M/O & 2142.76 & M/O\\\hline
    9 & !307.67 & M/O & 2203.45 & M/O & 971.01 & M/O & 4243.34 & M/O\\\hline
    10 & !558.34 & M/O & 7681.93 & M/O & 2274.30 & M/O & 7786.82 & M/O\\\hline
  \end{tabular}
  \caption{Run-times for searching for models (in secs).}
  \label{tab:qf-grabh}
\end{table}

%   \begin{tabular}[t]{|c|c|c|}\hline
%    \textbf{Size}  & {\textbf{Model B}}  &  {\textbf{Model E}} \\\hline
%    
%    2 & !0.09 & !0.12 \\\hline
%    3  & !0.54  & !0.75 \\\hline
%    4 &  !2.33 & !3.35 \\\hline
%    5 & !7.7 & !13.05 \\\hline
%    6 &  !20.05 & !40.64 \\\hline
%    7 & !51.86 & !152.78 \\\hline
%    8 & !112.24 &  !344.26 \\\hline
%    9 &  !236.31 & !880.73\\\hline
%    10 &  !531.56 &  !2133.89\\\hline
%  \end{tabular}
%  \caption{Run-times for searching for models (in secs).}
% % \label{tab:qf-grabh}
%\end{table} 

%\begin{table}[t]
%  \centering
%  \begin{tabular}[t]{|c|c|c|c|}\hline
%    \textbf{Size} &  \textbf{Model A}   & \textbf{Model B} &  \textbf{Model E} \\\hline
%   
%    2 & !0.0853381156921 & !0.091157913208 & !0.117037057877 \\\hline
%    3 & !0.540871858597 & !0.537098646164  & !0.754279375076 \\\hline
%    4 & !2.57536292076 & !2.33045578003 & !3.35159707069 \\\hline
%    5 & !7.70005106926 & !7.71436476707 & !13.0516757965 \\\hline
%    6 & !22.9898321629 & !20.0573630333 & !40.6696507931 \\\hline
%    7 & !57.0719909668 & !51.860738039 & !152.783704758 \\\hline
%    8 & !164.140100718 &  !112.248553038 &  !344.268831253 \\\hline
%    9 & !307.675467253 & !236.317871094 & !880.730427027\\\hline
%    10 & !558.342684269 &  !531.565055132 &  !2133.8986\\\hline
%  \end{tabular}
%  \caption{Runtimes for searching for models}
%  \label{tab:qf-grabh}
%\end{table}


%\begin{table}[t]
%  \centering
%  \begin{tabular}[t]{|c|c|c|c|}\hline
%    \textbf{Size} &  \textbf{Model A}   & \textbf{Model B} &  \textbf{Model E} \\\hline
%   
%    2 & !0.0853381156921 & !0.091157913208 & !0.117037057877 \\\hline
%    3 & !0.540871858597 & !0.537098646164  & !0.754279375076 \\\hline
%    4 & !2.57536292076 & !2.33045578003 & !3.35159707069 \\\hline
%    5 & !7.70005106926 & !7.71436476707 & !13.0516757965 \\\hline
%    6 & !22.9898321629 & !20.0573630333 & !40.6696507931 \\\hline
%    7 & !57.0719909668 & !51.860738039 & !152.783704758 \\\hline
%    8 & !164.140100718 &  !112.248553038 &  !344.268831253 \\\hline
%    9 & !307.675467253 & !236.317871094 & !880.730427027\\\hline
%    10 & !558.342684269 &  !531.565055132 &  !2133.8986\\\hline
%  \end{tabular}
%  \caption{Runtimes for searching for models}
%  \label{tab:qf-grabh}
%\end{table}

%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> v2-dia.tex <==
\begin{figure}
\centering

\begin{tikzpicture}[orm,every predicate/.style={}]
    \entity (E) {Node1\\($M_0 M_1 M_2 M_3 M_4$)};
    \binary[left=of E.north west, unique=2] (h) {};

       % \binary[left=of E.north west, unique=1-2] (w) {};

    \binary[left=of E.south west, unique=1-2](i) [below=6mm of h]{};
    \node[role name,
at=(i.north),anchor=south] {[$M_{0} M_{1} M_{3}$]};
    \plays[] (E) to (i.east);
   % \plays(h) to (i);
%         label=below:\ormleft{uses] (u) {};
\node[role name,
at=(h.north),anchor=south] {[$M_{0} M_{1}$]};

    \entity[left=of h] (Rank) {Node0\\($M_0 M_1 M_2 M_3 M_6$)};
  %  \entity[left=of u] (Car) {CompanyCar\\(.regNr)};
  

    \plays[mandatory] (E) to (h.east);
    \plays (h) to (Rank) (E);
    \plays[mandatory] (Rank) to (i.west);
    %to (u.east) (u) to (Car);


    \binary[right=of E.north east] (b) {};
    \node[role name,
at=(b.north),anchor=south] {[$M_{0} M_{1}$]};
       % \binary[right=of E.north east] (dd) {};

    \binary[right=of E.south east, unique,] (i) {};
    \node[role name,
at=(i.north),anchor=south] {[$M_{1} M_{2} M_{3}$]};
\binary[unique=1-2,skip unique=1-2] (xyz) [above=6mm of h] {};
% describes blue label above h Left uppermost
\node[role name,
at=(xyz.north),anchor=south] {[$M_{0} M_{1} M_{3}$]};
      
        
      \plays (Rank) to (xyz.west); 
    \plays[mandatory] (E) to (xyz.east);
      
    \entity[right=1.8 of E] (Date) {Node2\\($M_1 M_2 M_3 M_6 M_8$)};
   %\plays[mandatory] (E) to (xx.west); 

    \plays[mandatory] (E) to (b.west); 
    \plays (E) to (i.west);
    \plays (b.east) to (Date);
    \plays[mandatory] (Date) to (i.east);
    
%    \entity[label={[constraint]\#=$n$}] {E};
%\draw (Rank) to node[vroles,label=has,label=below:\ormup{of}]{} (E);
%\node[constraint,anchor=north west,inner ysep=0]
%at (h.) {\ormbraces{a, b, c}};
%\draw (E) to node[roles,
%label=below:drives]{} (Rank);

\node[roles=2][,unique=1-2,skip unique=2] (abc) [below=11mm of E] {};
\node[role name,
at=(abc.north),anchor=south] {[$M_{2} M_{3}$]};
\plays[mandatory] (Rank.south) -- (abc.west);  
\plays (abc.east) -- (Date.south);

  %  \node[role name, anchor=south west] at (b.east) {[birthdate]};
  %  \node[role name, anchor=north west] at (i.east) {[hiredate]};

%     \rules at (-.4, -2) {
%          \node[rule=1] {{$M_{2}$} $M_{3}$};\\
%      };
\end{tikzpicture}

\caption{Dia V2} \label{fig:v2}
\end{figure}

